Ontology-Guided Query Expansion for Biomedical Document Retrieval using Large Language Models

Effective Question Answering (QA) on large biomedical document collections requires effective document retrieval techniques. The latter remains a challenging task due to the domain-specific vocabulary and semantic ambiguity in user queries. We propose BMQExpander, a novel ontology-aware query expansion pipeline that combines medical knowledge - definitions and relationships - from the UMLS Metathesaurus with the generative capabilities of large language models (LLMs) to enhance retrieval effectiveness. We implemented several state-of-the-art baselines, including sparse and dense retrievers, query expansion methods, and biomedical-specific solutions. We show that BMQExpander has superior retrieval performance on three popular biomedical Information Retrieval (IR) benchmarks: NFCorpus, TREC-COVID, and SciFact - with improvements of up to 22.1% in NDCG@10 over sparse baselines and up to 6.5% over the strongest baseline. Further, BMQExpander generalizes robustly under query perturbation settings, in contrast to supervised baselines, achieving up to 15.7% improvement over the strongest baseline. As a side contribution, we publish our paraphrased benchmarks. Finally, our qualitative analysis shows that BMQExpander has fewer hallucinations compared to other LLM-based query expansion baselines.

==> sections/a_intro.tex <==
\section{Introduction}

Biomedical document querying is essential for supporting biomedical research and clinical decision-making. 
It helps doctors and researchers quickly find clinical guidelines, scientific studies, and the latest biomedical knowledge \cite{sivarajkumar2024clinical}.
Biomedical document retrieval is also a critical component in Question Answering (QA) or conversation QA pipelines \cite{qu2020open}.




%This improves patient care by supporting more informed and up-to-date decisions. When reliable medical information is built into tools like electronic health records (EHRs), it also makes daily clinical tasks easier and helps healthcare professionals work together more effectively \cite{sivarajkumar2024clinical}. 

However, retrieving relevant documents in response to a user query is challenging due to the complexity and potential ambiguity of biomedical language and terminology. Queries are often short, ambiguous, or lack precise terminology, which limits the effectiveness of traditional retrieval models \cite{almasri2016comparison}. Query expansion techniques have the potential to mitigate these challenges by augmenting the initial query with semantically related terms or phrases, thereby increasing recall and improving alignment between the user’s intent and the language used in relevant documents. These related terms can be derived from various sources, such as pseudo-relevance feedback based on top-ranked documents retrieved in an initial search, or generated using large language models (LLMs) capable of capturing contextual and domain-specific semantics \cite{wang2023query2doc}.

Recent advances in large language models (LLMs) have enabled significant progress in query understanding and expansion \cite{jagerman2023query, chen2024analyze}. Most existing query expansion methods employ LLM prompting and rely on the generalization capabilities of LLMs to generate additional context or reformulated queries.  
We argue that these methods are ineffective, especially for the semantically complex biomedical domain, due to the following reasons:

\begin{enumerate}
    \item \textbf{Factual unreliability and error propagation}: LLMs can generate plausible-sounding but inaccurate or fabricated biomedical terms during query expansion. These incorrect expansions may shift the original intent of the query or introduce clinically invalid terminology. When such expansions are passed to a retriever, they can lead to the retrieval of low-quality or irrelevant documents, ultimately propagating errors throughout the retrieval pipeline and compromising the reliability of downstream decision-making.

    \item \textbf{Model inconsistency and drift}: LLM-generated expansions are highly sensitive to the choice of model and prompt configuration. Different LLMs or even different versions of the same model can produce entirely different expansions for the same query. Minor changes in decoding parameters (e.g., temperature, top-$k$ sampling) or prompt wording can significantly alter expansion behavior, resulting in inconsistent retrieval outputs and making reproducibility a serious challenge in biomedical applications.

    \item \textbf{Computational inefficiency}: Generating expansions using LLMs can be resource-intensive, particularly when incorporating advanced prompting techniques such as few-shot learning, iterative refinement, or multi-stage pipelines \cite{chen2024analyze}. For example, retrieving top-ranked documents via a baseline retriever (pseudo-relevance feedback) and then using them to condition the LLM adds additional computational steps. Similarly, using multiple LLM calls for re-ranking, filtering, or refining queries can lead to substantial latency and cost, limiting scalability in practical applications.

    \item \textbf{Lack of interpretability and control}: LLM-based expansions are typically produced through opaque generation processes, with little visibility into why certain terms are included. This lack of interpretability is especially problematic in biomedical domains, where trust, safety, and explainability are critical. Without explicit grounding in trusted medical knowledge sources, it becomes difficult for practitioners to validate or audit the expanded terms, reducing confidence in the retrieval system and hindering effective analysis.



\end{enumerate}

These issues raise an important research question: \emph{Can we design a biomedical query expansion framework that reduces dependence on LLM generalization and instead leverages trusted, structured medical knowledge for generating context?}

In this paper, we propose a method that integrates structured biomedical ontologies with the generative abilities of LLMs in a controlled and interpretable way. Our approach is \textbf{LLM-agnostic} - the expansion is primarily driven by medical definitions and concept relationships retrieved from the \textbf{UMLS Metathesaurus}, rather than generated freely from the language model.

We begin by extracting key medical terms from a user query using an LLM guided by in-context examples. These terms are then mapped to medical concepts (CUIs) in UMLS. From these CUIs, we retrieve curated definitions and semantic relationships using well-established biomedical vocabularies (e.g., MeSH, SNOMED, NCI). We then build a pruned semantic graph using a simple heuristic that selects edges based on domain-specific relevance to represent relevant concept hierarchies and associations. This structured information is serialized and used as input to an LLM, which is prompted to generate a pseudo-document, which is a medically grounded, context-rich response to the original query. Finally, we expand the query by combining the original input with the LLM’s grounded output and perform retrieval using a standard ranking function.

This leads us to a second research question: \emph{Can the integration of rich, structured medical ontologies improve the reliability and semantic fidelity of LLM-generated expansions while preserving flexibility across model choices?}

Our method answers this by combining symbolic and neural reasoning: we use symbolic knowledge from UMLS to constrain and inform the language model, guiding it to generate expansions that are both semantically faithful and medically valid. This design minimizes hallucination, supports reproducibility, and enables generalization across LLM variants.

To summarize, the main contributions of this paper are:
{\color{red}
\begin{itemize}
    \item We propose a novel LLM-agnostic query expansion framework that uses medical knowledge from UMLS to generate grounded, context-rich expansions.
    \item We introduce a concept-level semantic graph construction method that captures curated hierarchical and associative relationships among medical concepts linked to the query. The graph is pruned to retain only highly relevant UMLS relations and then serialized into a structured textual representation, which serves as grounded biomedical context for the LLM to generate reliable query expansions.
%    \item We show how structured biomedical information can be used to prompt LLMs in a constrained way, mitigating hallucination while preserving flexibility and effectiveness.
    \item We created and published new biomedical retrieval dataset by perturbing the queries in the original dataset. This allows us to reveal weaknesses in previous retrieval methods that rely on extensive training data.
    
    \item We implemented a wide range of biomedical document retrieval baselines, including query expansion methods, LLM prompting approaches, and both dense and sparse retrieval models. Furthermore, we show that our method generalizes well across both open and closed-source large language models.
    
    \item We perform extensive experiments on three benchmark datasets and show that our method achieves competitive performance. Our method also demonstrates strong generalization under query perturbations, and significant reduction in hallucinations, making it highly effective and reliable for biomedical information retrieval.
\end{itemize}
}

The remainder of the paper is organized as follows. Section 2 reviews related work. Section 3 details our proposed methodology. Section 4 introduces our dataset contribution. Section 5 describes the experimental setup and presents the results. Finally, Section 6 concludes the paper.


==> sections/c_methodology.tex <==
\section{Methodology}

Let $\mathcal{Q}$ be the space of user queries and $\mathcal{D}$ the corpus of biomedical documents. Given a query $q \in \mathcal{Q}$, our objective is to construct a medically enriched, semantically faithful expanded query $q' \in \mathcal{Q}'$ such that retrieval with $q'$ yields improved retrieval performance and robustness compared to using $q$ directly.

We propose a five-stage pipeline,

\begin{enumerate}
    \item Domain-Specific Entity Recognition
    \item Ontology-Driven Concept Linking and Definition Retrieval
    \item Concept-Level Knowledge Graph Construction
    \item Ontology-Guided Pseudo-document generation %Contextualized Generation Guided by Biomedical Ontology
    \item Weighted Query Expansion and Retrieval
\end{enumerate}



\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Ontology_Method_Diagram.pdf}
    \caption{Schematic diagram of the proposed method. Here, $c3$ represents CUI C0029118.}
    \label{fig:proposed_method}
\end{figure*}





\subsection{Domain-Specific Entity Recognition}


We begin by identifying key biomedical terms in a user query $q \in \mathcal{Q}$. Let $\mathcal{V}$ denote the vocabulary of biomedical concepts. We define an entity recognition function,

\[
\mathcal{T} : \mathcal{Q} \rightarrow 2^{\mathcal{V}}
\]

that maps a query to a subset of biomedical terms $T_q$.

\[
T_q = \mathcal{T}\left(q\right) \subseteq \mathcal{V}, \quad T_q = \{ t_1, t_2, \ldots, t_n \}
\]

The function $\mathcal{T}$ is instantiated via few-shot prompting of a large language model (LLM) using curated in-context examples. This enables recognition of implicitly or semantically expressed biomedical terms beyond string-matching. If the model determines that no medically meaningful terms are present, we assign $T_q = \emptyset$.












\subsection{Ontology-Driven Concept Linking and Definition Retrieval}


\subsubsection{Concept Linking via UMLS Search}

Following biomedical term extraction, we link each identified term $t_i \in T_q$ to its corresponding Concept Unique Identifier (CUI) $c_i$ using the UMLS Metathesaurus. Let $\mathcal{CUI}$ denote the space of CUIs. We define a concept normalization function that maps each biomedical term to a corresponding CUI.

\[
\mathcal{C} : \mathcal{V} \rightarrow \mathcal{CUI}
\]

 We then define the set of CUIs for a given query as,

\[
C_q = \{ \mathcal{C}\left(t_i\right) \mid t_i \in T_q \} = \{ c_1, c_2, \ldots, c_n \}
\]

To resolve each term $t_i \in T_q$ to its corresponding Concept Unique Identifier (CUI) $c_i \in \mathcal{CUI}$, we query the UMLS Metathesaurus using an exact-match search strategy. Specifically, we use the UMLS API\footnote{\url{https://documentation.uts.nlm.nih.gov/rest/home.html}} to perform concept lookups, requiring that the returned concept exactly matches the lexical form of $t_i$ to avoid the noise and ambiguity often introduced by partial or fuzzy matching.

If the exact-match search returns multiple CUIs for a term, we select the top concept and retrieve its identifier. Terms with no exact match are discarded to prevent erroneous mappings and preserve semantic precision. The resulting set of CUIs, $C_q$, provides a structured representation of the query, enabling accurate alignment with biomedical ontologies in subsequent retrieval stages.



\subsubsection{Definition Retrieval}


Each CUI $c_i \in C_q$ is associated with one or more definitions retrieved from UMLS. We source the definitions from a set of curated biomedical vocabularies,

\[
\mathbb{S} = \{ \text{MSH}, \text{SNOMEDCT\_US}, \text{NCI}, \text{CSP} \}
\]

Here, \texttt{MSH} denotes the \textit{Medical Subject Headings (MeSH)}, \texttt{SNOMEDCT\_US} indicates the \textit{Systematized Nomenclature of Medicine Clinical Terms, US Edition}, \texttt{NCI} refers to the \textit{National Cancer Institute Thesaurus}, and \texttt{CSP} corresponds to the \textit{CRISP Thesaurus}. We restrict definition retrieval to these four vocabularies, as they consistently provide concise, well-structured definitions and offer better coverage across our evaluation datasets which is supported by \cite{zivaljevic2022utility}.


For each concept $c_i \in C_q$, we retrieve definitions from curated biomedical vocabularies. Each definition is paired with its provenance to maintain semantic transparency. Formally, we define the definition set for a concept $c_i$ as,

\[
D_i = \left\{ (d_{ij}, s_{ij}) \;\middle|\; d_{ij} \in \mathbb{D},\; s_{ij} \in \mathbb{S},\; j = 1, \ldots, k_i \right\}
\]

where $d_{ij}$ is a natural language definition and $s_{ij}$ is the source vocabulary (e.g., \texttt{MSH}, \texttt{NCI}, \texttt{SNOMEDCT\_US}, \texttt{CSP}) from which it was retrieved. 

To ensure clarity and consistency during downstream prompting, we serialize all definitions for a given concept $c_i$ into a single structured string. Each entry follows the below format,

%\begin{tcolorbox}[colback=gray!5, colframe=black!60, boxrule=0.4pt, arc=2pt, fontupper=\ttfamily\small, title=Serialized Definition Representation]
%[Concept Name]: definition$_1$ (Source: Vocabulary$_1$); definition$_2$ (Source: Vocabulary$_2$); $\ldots$; definition$_k$ (Source: Vocabulary$_k$)
%\end{tcolorbox}



\begin{tcolorbox}[
  colback=gray!5,
  colframe=black!60,
  boxrule=0.4pt,
  arc=2pt,
  enhanced,
  title=Definition Template,
  left=4pt, right=4pt, top=4pt, bottom=4pt,
]

% Schema box
\begin{tcolorbox}[
  colback=white,
  colframe=black!40,
  boxrule=0.2pt,
  sharp corners,
  left=4pt, right=4pt, top=2pt, bottom=2pt,
  title=\textbf{\sffamily Template},
  fonttitle=\bfseries\sffamily\scriptsize,
  fontupper=\ttfamily\footnotesize,
  enhanced
]
[\textit{Concept Name}]: definition$_1$ (Source: Vocabulary$_1$); definition$_2$ (Source: Vocabulary$_2$); $\ldots$ definition$_k$ (Source: Vocabulary$_k$);
\end{tcolorbox}

\vspace{4pt}

% Example box
\begin{tcolorbox}[
  colback=white,
  colframe=black!40,
  boxrule=0.2pt,
  sharp corners,
  left=4pt, right=4pt, top=2pt, bottom=2pt,
  title=\textbf{\sffamily Example},
  fonttitle=\bfseries\sffamily\scriptsize,
  fontupper=\ttfamily\footnotesize,
  enhanced
]
Type 1 Diabetes: subtype of diabetes mellitus that is characterized by insulin deficiency; it is manifested by the sudden onset of severe hyperglycemia, rapid progression to diabetic ketoacidosis, and death unless treated with insulin; the disease may occur at any age, but is most common in childhood or adolescence. (Source: CRISP Thesaurus); A subtype of DIABETES MELLITUS that is characterized by INSULIN deficiency. It is manifested by the sudden onset of severe HYPERGLYCEMIA, rapid progression to DIABETIC KETOACIDOSIS, and DEATH unless treated with insulin. The disease may occur at any age, but is most common in childhood or adolescence. (Source: MeSH); A chronic condition characterized by minimal or absent production of insulin by the pancreas. (Source: National Cancer Institute (NCI) Thesaurus); 
\end{tcolorbox}

\end{tcolorbox}



This format allows multiple definitions to be combined in a readable way while preserving the source of each. By linking each concept to trusted biomedical vocabularies, it is expected to help reduce ambiguity and mitigate hallucination in downstream generation \cite{huang2023citation, byun2024reference}.




\subsection{Concept-Level Knowledge Graph Construction}

To enrich each query with structured biomedical knowledge, we construct a graph over the CUIs linked from the extracted terms. Let $C_q = \{c_1, c_2, \ldots, c_n\}$ denote the set of CUIs associated with query $q$. We define a directed labeled graph $G_q = (V_q, E_q)$, where the node set is $V_q = C_q$ and each edge $(c_i, c_j, r) \in E_q$ represents a semantic relation $r \in \mathcal{R}$ between concepts $c_i$ and $c_j$ as defined in the UMLS Metathesaurus.

Since UMLS contains a large and heterogeneous set of relation types, many of which are either overly broad or semantically redundant for biomedical retrieval, we prune the relation set using a filtering function,

\[
\phi_{\text{prune}} : \mathcal{R} \rightarrow \{0,1\}
\]

that retains only medically meaningful relations:

\[
\mathcal{R}' = \left\{ r \in \mathcal{R} \;\middle|\; \phi_{\text{prune}}(r) = 1 \right\}
\]

\[
= \{ \texttt{CHD},\ \texttt{PAR},\ \texttt{SY},\ \texttt{RO},\ \texttt{RO:has\_associated\_morphology} \}
\]



\texttt{CHD} (has child) and \texttt{PAR} (has parent) capture hierarchical \textit{is-a} relationships useful for modeling taxonomic structures; 
\texttt{SY} (synonym) links conceptually equivalent terms, aiding in synonym-aware retrieval; 
\texttt{RO} (related other) expresses general associative relationships; and 
\texttt{RO : has\_associated\_morphology} is a specific subrelation indicating morphological associations (e.g., linking a disease to its pathological form). 

Applying this filter, we obtain a pruned edge set,

\[
E_q' = \left\{ (c_i, c_j, r) \in E_q \;\middle|\; r \in \mathcal{R}' \right\}, \quad \text{yielding} \quad G_q' = (V_q, E_q')
\]

This pruning removes weak or noisy edges, improving the interpretability and reliability of the resulting graph. 

To make $G_q'$ consumable by large language models, we serialize it into a textual form $S_q \in \mathcal{T}_{\text{text}}$. Each node $c_i \in V_q$ is represented by its outgoing edges in a hierarchical, indented format:




\begin{tcolorbox}[colback=green!5, colframe=gray!80!black, arc=2pt, boxrule=0.3pt, title=Serialized Relational Representation, fontupper=\ttfamily\small]
Carcinoma of breast: \\
\hspace*{1em} $\llcorner$ has parent: Infiltrating duct carcinoma \\
\hspace*{1em} $\llcorner$ is synonymous with: Breast cancer
\end{tcolorbox}


This textual format retains the semantic integrity of the ontology while making the relational structure directly usable in language model prompts. By encoding only high-confidence, ontology-backed links, it reduces ambiguity and helps prevent hallucinations during generation. This ensures that the expanded queries remain medically grounded and aligned with the intended biomedical context.


\subsection{Contextualized Generation Guided by Biomedical Ontology}

To generate a semantically enriched pseudo-document $p_q$, we define a grounded generation function,

%\[
%\mathcal{G} : \mathcal{Q} \times \mathcal{D}_q \times %\mathcal{T}_{\text{text}} \rightarrow \mathcal{P}
%\]

\[
\mathcal{G} : \mathcal{Q} \times \mathcal{D}_q \times \mathcal{S} \rightarrow \mathcal{P}
\]

\[
p_q = \mathcal{G}\bigl(q,\ \mathcal{D}_q,\ S_q\bigr)
\]

% $S_q \in \mathcal{T}_{\text{text}}$ is the serialized relational context\textbf{}

Here, $\mathcal{Q}$ denotes the space of user queries, $\mathcal{D}_q$ is the set of structured definitions retrieved for the query-specific concepts, and $S_q$ is the serialized relational context derived from the ontology-pruned concept graph. The output space $\mathcal{P} \subset \Sigma^*$ denotes the set of natural language pseudo-documents.

We prompt a large language model (LLM) with three components: the original query $q$, the definition set $\mathcal{D}_q$, and the serialized relational structure $S_q$. The prompt is formatted as:

\begin{verbatim}
Query: [q]
Definitions: [definitions]
Relationships: [relationships]
\end{verbatim}

Furthermore, we append a chain-of-thought suffix (e.g., “Give the rationale before answering.”) to encourage step-by-step reasoning in the generated output.

While the model may incorporate prior knowledge from pretraining, constraining its context to trusted, UMLS-derived definitions and relations provides strong semantic guidance. This helps reduce hallucination and ensures biomedical relevance, especially under paraphrased or underspecified queries.


\subsection{Weighted Query Expansion and Retrieval}

To form the final expanded query, we combine the original query $q \in \mathcal{Q}$ with the pseudo-document $p_q$ generated by the language model. We define the expanded query $q' \in \mathcal{Q}'$ as,

\[
q' = \underbrace{q \oplus q \oplus \cdots \oplus q}_{\alpha\ \text{times}} \oplus\ p_q
\]

where $\oplus$ denotes string concatenation, and the weighting factor $\alpha = 5$ controls the relative influence of the original query versus the generated content. 

We use the BM25 retrieval model to rank documents in the corpus $\mathcal{D}$ based on the expanded query $q'$. This formulation boosts term frequency for original query terms while introducing medically grounded expansions through $p_q$.




\begin{figure}[ht]
    \centering
    % First subfigure - full KG
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{kg_before.pdf}
        \caption{Full Knowledge Graph}
        \label{fig:kg-before}
    \end{subfigure}
    \hfill
    % Second subfigure - pruned KG
    \begin{subfigure}[t]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{pruned_kg.pdf}
        \caption{Pruned Knowledge Graph}
        \label{fig:pruned-kg}
    \end{subfigure}
    
    \caption{Comparison of the full and pruned knowledge graphs.}
    \label{fig:kg-comparison}
\end{figure}





==> sections/d_datasets.tex <==
\section{Datasets}


We evaluate our method on three widely-used benchmarks in biomedical information retrieval: \textbf{NFCorpus}, \textbf{SciFact}, and \textbf{TREC-COVID}. These datasets vary in query intent, document complexity, and domain specificity, providing a comprehensive evaluation environment.

\subsection{Benchmark Datasets}
\paragraph{NFCorpus.} 
NFCorpus is a full-text medical information retrieval dataset containing 3,244 natural language queries harvested from NutritionFacts.org. The queries are non-technical and user-oriented, whereas the associated documents—drawn primarily from PubMed—are technical and terminology-heavy. It includes over 9,000 medical documents and nearly 170,000 relevance judgments, with query-document links established via a hierarchy of citation strength. The dataset is split into training (80\%), development (10\%), and testing (10\%) based on query-level partitions.

\paragraph{SciFact.} 
SciFact is a scientific fact-checking benchmark comprising 1,400 expert-written scientific claims paired with biomedical abstracts. Each claim is annotated with supporting or refuting evidence, along with sentence-level rationales. The dataset includes a separate corpus of abstracts with document IDs and metadata. Queries in SciFact are formal claims rather than keyword-style questions, enabling assessment of semantic retrieval capabilities and evidence-grounded reasoning.

\paragraph{TREC-COVID.}
TREC-COVID is a large-scale ad hoc retrieval dataset built on the CORD-19 corpus, a continuously updated collection of scientific articles on COVID-19. Structured over five rounds, the dataset includes hundreds of expert-formulated information needs (topics) and human-annotated relevance judgments. TREC-COVID evaluates the ability of systems to retrieve relevant literature in response to urgent, evolving biomedical questions—reflecting real-world use in dynamic public health crises.

\subsection{Query Perturbation and Paraphrased Datasets}

Many biomedical retrievers exhibit sensitivity to variations in query wording, which reduces their effectiveness when users express similar information needs differently. To evaluate robustness under query paraphrasing, we create three paraphrased versions of the original benchmarks: \textbf{NFCorpus-P}, \textbf{SciFact-P}, and \textbf{TREC-COVID-P}.

We use \textbf{GPT-4o} to generate paraphrased queries. For each original query, we apply the following prompt:

\begin{quote}
\texttt{Paraphrase the following query.} \\
\texttt{Query: [query]} \\
\texttt{Paraphrased query:}
\end{quote}

This approach preserves the intent and relevance structure of the original datasets while introducing natural lexical and syntactic variation. The resulting paraphrased benchmarks allow us to measure how well retrieval systems generalize to diverse phrasings, simulating realistic query reformulations encountered in user interactions.



\begin{table*}[ht]
    \centering
    \scriptsize
    \caption{Dataset statistics and query samples}
    \renewcommand{\arraystretch}{1.2} % increase row height slightly
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{
        |l
        |c
        |c
        |c
        |c
        |c
        |>{\hspace{2pt}}p{5.8cm}<{\hspace{2pt}}
        |>{\hspace{2pt}}p{5.8cm}<{\hspace{2pt}}|
    }
        \hline
        \textbf{Dataset} 
        & \textbf{\# Docs} 
        & \textbf{\# Queries} 
        & \textbf{Avg. Doc Length} 
        & \textbf{Avg. Query Length} 
        & \textbf{\# Unique Words} 
        & \textbf{Original Query Example} 
        & \textbf{Paraphrased Query Example} \\
        \hline

        \multirow{3}{*}{NFCorpus-P} 
        & \multirow{3}{*}{3,633} 
        & \multirow{3}{*}{323} 
        & \multirow{3}{*}{219.656} 
        & \multirow{3}{*}{5.344} 
        & \multirow{3}{*}{36,735} 
        & Cancer Risk From CT Scan Radiation 
        & Risk of Developing Cancer Due to Radiation from CT Scans \\
        \cline{7-8}
        & & & & & 
        & BPH 
        & What is benign prostatic hyperplasia? \\
        \cline{7-8}
        & & & & & 
        & Preventing Brain Loss with B Vitamins? 
        & Can B vitamins help stop brain deterioration? \\
        \hline

        \multirow{3}{*}{TREC-COVID-P} 
        & \multirow{3}{*}{1,71,332} 
        & \multirow{3}{*}{50} 
        & \multirow{3}{*}{148.192} 
        & \multirow{3}{*}{11.860} 
        & \multirow{3}{*}{3,83,990} 
        & what causes death from Covid-19? 
        & What factors lead to fatalities in Covid-19 cases? \\
        \cline{7-8}
        & & & & & 
        & What is the mechanism of cytokine storm syndrome on the COVID-19? 
        & How does a cytokine storm occur in COVID-19 patients? \\
        \cline{7-8}
        & & & & & 
        & Does Vitamin D impact COVID-19 prevention and treatment? 
        & Can Vitamin D affect the prevention and treatment of COVID-19? \\
        \hline

        \multirow{3}{*}{SciFact-P} 
        & \multirow{3}{*}{5,183} 
        & \multirow{3}{*}{300} 
        & \multirow{3}{*}{200.811} 
        & \multirow{3}{*}{14.630} 
        & \multirow{3}{*}{50,571} 
        & DMRT1 is a sex-determining gene that is epigenetically regulated by the MHM region. 
        & The MHM region regulates the DMRT1 gene, which plays a role in sex determination, through epigenetic mechanisms. \\
        \cline{7-8}
        & & & & & 
        & Birth-weight is positively associated with breast cancer. 
        & Higher birth-weight is linked to an increased risk of breast cancer. \\
        \cline{7-8}
        & & & & & 
        & High levels of copeptin decrease risk of diabetes. 
        & Elevated copeptin levels lower the risk of developing diabetes. \\
        \hline
    \end{tabular}
    }
    \label{tab:dataset_stats_queries}
\end{table*}







==> sections/e_experiments.tex <==
\section{Experiments}




We evaluate our proposed method across three benchmark biomedical retrieval datasets: \textbf{NFCorpus}, \textbf{TREC-COVID}, and \textbf{SciFact}. The goal is to retrieve and rank relevant documents given a query. We primarily report \textbf{NDCG@10} as our main evaluation metric. For LLM-based comparisons and evaluations on paraphrased datasets (e.g., NFCorpus-P, SciFact-P), we also report \textbf{mAP@10} and \textbf{Recall@10} to provide a more comprehensive view of performance.

\subsection{Experimental Setup}

\paragraph{MetaMap Definitions.}
We implement a query expansion baseline inspired by prior work using metamap and biomedical ontologies for retrieval improvement \cite{di2019exploring}. Specifically, we use MetaMap to extract medical concepts from queries, restricting to selected semantic types to ensure relevance (\texttt{dsyn} (Disease or Syndrome), \texttt{sosy} (Sign or Symptom), etc.). For each extracted concept, we retrieve its definition from the UMLS Metathesaurus, constraining the selection to definitions provided by the SNOMED CT (\texttt{SNOMEDCT\_US}), MeSH (\texttt{MSH}), National Cancer Institute Thesaurus (\texttt{NCI}), and CRISP Thesaurus (\texttt{CSP}) vocabularies.
The expanded query is formed by repeating the original query with a weight of $\alpha = 10$ and concatenating the retrieved definitions with a weight of $1$, maintaining a strong emphasis on the original user intent similar to \cite{di2019exploring}. Retrieval is performed using BM25.


\subsection{Main Experiment}

Table~\ref{tab:ndcg_comparison} presents the NDCG@10 scores of our method compared to a range of baselines, including traditional sparse retrievers, query expansion methods, and recent dense retrievers. We include biomedical concept-based methods (MetaMap +UMLS), simple query expansion (Query2Doc), and strong dense models such as \textbf{Contriever}, \textbf{Dragon}, \textbf{SPECTER 2.0}, and instruction-tuned retrievers like \textbf{SGPT}, \textbf{MedCPT}, and \textbf{BMRetriever-410M}. BM25 serves as the sparse baseline. 

Our method achieves the highest NDCG@10 on \textbf{NFCorpus} (0.363), outperforming strong baselines such as MedCPT (0.340) and InstructOR-L (0.341). On \textbf{TREC-COVID}, it reaches 0.801, closely trailing BMRetriever-410M (0.831) and outperforming Dragon (0.759). For \textbf{SciFact}, we report 0.704, which is competitive with MedCPT (0.724).

These results demonstrate that our method performs consistently well across datasets with different biomedical content and query styles.

\subsection{Query Perturbation Experiment}

Table~\ref{tab:perturbed_methods} presents the retrieval performance of various methods on paraphrased versions of three benchmark datasets—NFCorpus-P, TREC-COVID-P, and SciFact-P—designed to evaluate robustness under query perturbation. We report standard retrieval metrics including NDCG@10, mAP@10, and Recall@10. Among the baselines, Contriever and MedCPT show relatively strong performance, while BMRet-410 and InstructOR demonstrate lower robustness, particularly on NFCorpus-P. Notably, our method (\textbf{Ours}\footnotemark), which combines retrieval with prompting-based semantic expansion, consistently achieves the best NDCG@10 across all datasets. On TREC-COVID-P, it surpasses the second-best method by a significant margin (+6.8 NDCG@10 over BMRet-410), while maintaining strong generalization on SciFact-P and NFCorpus-P. These results confirm that our approach remains highly effective even when the input queries are semantically altered, demonstrating both precision and resilience in noisy or rephrased query settings.




{\tiny
\renewcommand{\arraystretch}{1.4} % increase vertical spacing slightly
\begin{table}[ht]
    \caption{Comparison of NDCG@10 across datasets}
    \label{tab:ndcg_comparison}
    \centering
    \begin{adjustbox}{max width=\textwidth}
    \begin{tabular}{
        | >{\hspace{4pt}}l<{\hspace{4pt}} 
        | >{\hspace{4pt}}c<{\hspace{4pt}} 
        | >{\hspace{4pt}}c<{\hspace{4pt}} 
        | >{\hspace{4pt}}c<{\hspace{4pt}} |
    }
        \hline
        \multirow{2}{*}{\textbf{Method}} 
        & \multicolumn{3}{c|}{\textbf{Dataset}} \\
        \cline{2-4}
        & \textbf{NFCorpus} 
        & \textbf{TREC-COVID} 
        & \textbf{SciFact} \\
        \hline
        BM25\tablefootnote{\label{fn:bm25}We use the Pyserini BM25 implementation. URL: \url{https://github.com/castorini/pyserini}}             &   0.325    &   0.656    &   0.665   \\
        \hline
        Metamap Definitions \cite{di2019exploring}   &   0.330    &  0.637   &  0.667     \\
        \hline
        Query2Doc \cite{wang2023query2doc}      & 0.303      &  0.651     &       \\
        \hline
        CSQE       & -      &  0.742     &  0.696      \\
        \hline
        Contriever \cite{izacard2021unsupervised}      &   0.328    &   0.596    &  0.677     \\
        \hline
        Dragon  \cite{lin2023train}     &  0.339     &  \underline{0.759}     & 0.679      \\
        \hline
        SPECTER 2.0 \cite{singh2022scirepeval}     &   0.228    &    0.584   &   0.671    \\
  
  %      \hline
  %      SciMult \cite{zhang2023pre}         &   0.308    &   0.712    & 0.707  %     \\
  %      \hline
  %      COCO-DR    \cite{yu2022coco}      &  \underline{0.355}     &  0.789     &  0.709     \\
  
        
        \hline
        SGPT-1.3B \cite{muennighoff2022sgpt}        &   0.320    &   0.730    &  0.682     \\
        \hline
        MedCPT  \cite{jin2023medcpt}       &   \underline{0.340}    &  0.697     &  0.724     \\
        \hline
        GTR-L \cite{ni2021large}         &  0.329     &  0.557     & 0.639      \\
        \hline
        InstructOR-L \cite{su2022one}    &   \underline{0.341}    &  0.581     &  0.643     \\
        \hline
        BMRetriever-410M \cite{xu2024bmretriever}      &    0.321   &   \underline{0.831}    &  0.711     \\
        \hline
        \textbf{Ours}    &   \underline{0.363}    &  \underline{0.801}     & 0.704      \\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}
}

%\footnotetext[1]{We use the Pyserini BM25 %implementation. URL: %\url{https://github.com/castorini/pyserini%}}
    



\subsection{Evaluation of LLM Backbones}

Table~\ref{tab:metric_comparison} examines how different prompting strategies impact retrieval performance when using large language models (LLMs). We test \textit{zero-shot} and \textit{chain-of-thought (CoT)} prompting for multiple LLMs, including \textbf{LLaMA}, \textbf{GPT-4 Omni}, \textbf{Gemini 1.5}, and \textbf{Qwen}.

For example, using LLaMA in a zero-shot setting already outperforms BM25 across all datasets, with strong performance on \textbf{TREC-COVID} (NDCG@10 = 0.734) and \textbf{SciFact} (NDCG@10 = 0.695). CoT prompting further improves the NDCG@10 on NFCorpus from 0.353 to 0.359, showing that structured prompting can help extract more useful signal from LLMs. However, we also observe cases where CoT offers limited or no benefit, suggesting the effect of prompting is model- and dataset-specific.



These comparisons highlight the importance of prompt design when adapting general-purpose LLMs for biomedical search.






\begin{table*}[ht]
\caption{Performance on Query Perturbation (Paraphrased) Datasets across Retrieval Methods}
\label{tab:perturbed_methods}
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|l||ccc||ccc||ccc|}
\hline
\multirow{2}{*}{\textbf{Method}} 
& \multicolumn{3}{c||}{\textbf{NFCorpus-P}} 
& \multicolumn{3}{c||}{\textbf{TREC-COVID-P}} 
& \multicolumn{3}{c|}{\textbf{SciFact-P}} \\
\cline{2-10}
& \textbf{NDCG@10} & \textbf{mAP@10} & \textbf{Recall@10}
& \textbf{NDCG@10} & \textbf{mAP@10} & \textbf{Recall@10}
& \textbf{NDCG@10} & \textbf{mAP@10} & \textbf{Recall@10} \\
\hline
BMRet-410     & 0.245 & 0.083 & 0.119 & 0.606 & 0.016 & 0.018 & 0.677 & 0.632 & 0.801 \\
\hline
MedCPT        & 0.272 & 0.092 & 0.130 & 0.445 & 0.010 & 0.013 & 0.661 & 0.606 & 0.815 \\
\hline
Contriever    & 0.288 & 0.101 & 0.137 & 0.453 & 0.010 & 0.013 & 0.675 & 0.626 & 0.812 \\
\hline
InstructOR    & 0.291 & 0.096 & 0.139 & 0.437     & 0.009 & 0.011 & 0.623 & 0.576 & 0.752 \\
\hline
Query2Doc     & -       & - & - & -       & - & - & -       & - & - \\
\hline
\textbf{Ours} & \textbf{0.342} & \textbf{0.126} & \textbf{0.171} & \textbf{0.709} & \textbf{0.018} & \textbf{0.020} & \textbf{0.705} & \textbf{0.655} & \textbf{0.842} \\
\hline
\end{tabular}
\end{adjustbox}
%\footnotetext{We report our best %performance across prompting %variants.}
\end{table*}




\begin{table}[ht]
\caption{Ablation Study}
\label{tab:ablation_single}
\centering
\scriptsize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{|l||c|c|c|}
\hline
\textbf{Configuration} & \textbf{NDCG@10} & \textbf{mAP@10} & \textbf{Recall@10} \\
\cdashline{1-4}[2pt/1pt]
\textbf{BM25 Baseline} & 0.656 & 0.016 & 0.018 \\
\cdashline{1-4}[2pt/1pt]
w/o LLM & 0.701 & 0.018 & 0.019 \\
Definitions Only & 0.750 & 0.019 & 0.021 \\
Relations Only & 0.779 & 0.020 & 0.022 \\
Definitions + Relations & \underline{\boldmath 0.801} & \underline{\boldmath 0.021} & \underline{\boldmath 0.023} \\
\hline
\end{tabular}
\end{table}






\begin{table*}[ht]
\caption{Performance Comparison across Models and Prompting Strategies}
\label{tab:metric_comparison}
\centering
\scriptsize
\begin{adjustbox}{max width=\textwidth}
\setlength{\tabcolsep}{6pt}  % default is 6pt; increase for more horizontal padding
\renewcommand{\arraystretch}{1.3}  % increase row height
\begin{tabular}{|l|l||c|c|c||c|c|c||c|c|c|}
\hline
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Prompting}} 
& \multicolumn{3}{c||}{\textbf{NFCorpus}} 
& \multicolumn{3}{c||}{\textbf{TREC-COVID}} 
& \multicolumn{3}{c|}{\textbf{SciFact}} \\
\cline{3-11}
 & & \textbf{NDCG@10} & \textbf{mAP@10} & \textbf{Recall@10} 
   & \textbf{NDCG@10} & \textbf{mAP@10} & \textbf{Recall@10} 
   & \textbf{NDCG@10} & \textbf{mAP@10} & \textbf{Recall@10} \\
%\hline
\cdashline{1-11}[2pt/1pt]  % top dashed line
\multicolumn{2}{|c||}{\textbf{BM25 Baseline}} 
  & 0.325 & 0.124 & 0.157 & 0.656 & 0.016 & 0.018 & 0.665 & 0.616 & 0.799 \\
\cdashline{1-11}[2pt/1pt]
\multirow{2}{*}{LLaMA 3.1 8B} 
  & Zero Shot & 0.353 & 0.138 & 0.182 & 0.734 & 0.019 & 0.021 & 0.695 & 0.642 & 0.844  \\
\cline{2-11}
  & CoT       & 0.359 & 0.140 & 0.183 & 0.763 & 0.020 & 0.022 & 0.695 & 0.646 & 0.826 \\
\hline
\multirow{2}{*}{Qwen 2.5 32B} 
  & Zero Shot & 0.360 & 0.141 & 0.178 & 0.748 & 0.019 & 0.021 & 0.701 & 0.653 & 0.830  \\
\cline{2-11}
  & CoT       & 0.358 & 0.136  & 0.179 & 0.760 & 0.019 & 0.021 & \underline{\boldmath 0.707} & 0.658 & 0.837 \\
\hline
\multirow{2}{*}{DeepSeek-V3} 
  & Zero Shot & \underline{\boldmath 0.369} & 0.144 & 0.188  & 0.781 & 0.020  & 0.022  & 0.716 & 0.666 & 0.854 \\
\cline{2-11}
  & CoT       & 0.365 & 0.142 & 0.184 & \underline{\boldmath 0.800}  & 0.021 & 0.022 & \underline{\boldmath 0.723} & 0.675 & 0.857 \\
\hline
\multirow{2}{*}{Gemini 1.5 Pro} 
  & Zero Shot & 0.360 & 0.140 & 0.181 & 0.764 & 0.020 & 0.022 & 0.705 & 0.659 & 0.832 \\
\cline{2-11}
  & CoT       & 0.361 & 0.140 & 0.181 & 0.771 & 0.020 & 0.028 & 0.695 & 0.646 & 0.829 \\
\hline

\multirow{2}{*}{GPT-4 Omni} 
  & Zero Shot & \underline{\boldmath 0.365} & 0.143 & 0.187 & 0.785  & 0.020 & 0.022 & 0.700 & 0.649 & 0.838 \\
\cline{2-11}
  & CoT       & 0.363  & 0.141 & 0.181 & \underline{\boldmath 0.801}  & 0.021 & 0.023 & 0.704 & 0.654 & 0.845 \\
\hline


\end{tabular}
\end{adjustbox}
\end{table*}








==> sections/f_conclusion.tex <==
\section{Conclusion}
